Random Expert Sampling for Deep Learning Segmentation of Acute Ischemic Stroke on Non-contrast CT

Purpose: Multi-expert deep learning training methods to automatically quantify ischemic brain tissue on Non-Contrast CT Materials and Methods: The data set consisted of 260 Non-Contrast CTs from 233 patients of acute ischemic stroke patients recruited in the DEFUSE 3 trial. A benchmark U-Net was trained on the reference annotations of three experienced neuroradiologists to segment ischemic brain tissue using majority vote and random expert sampling training schemes. We used a one-sided Wilcoxon signed-rank test on a set of segmentation metrics to compare bootstrapped point estimates of the training schemes with the inter-expert agreement and ratio of variance for consistency analysis. We further compare volumes with the 24h-follow-up DWI (final infarct core) in the patient subgroup with full reperfusion and we test volumes for correlation to the clinical outcome (mRS after 30 and 90 days) with the Spearman method. Results: Random expert sampling leads to a model that shows better agreement with experts than experts agree among themselves and better agreement than the agreement between experts and a majority-vote model performance (Surface Dice at Tolerance 5mm improvement of 61% to 0.70 +- 0.03 and Dice improvement of 25% to 0.50 +- 0.04). The model-based predicted volume similarly estimated the final infarct volume and correlated better to the clinical outcome than CT perfusion. Conclusion: A model trained on random expert sampling can identify the presence and location of acute ischemic brain tissue on Non-Contrast CT similar to CT perfusion and with better consistency than experts. This may further secure the selection of patients eligible for endovascular treatment in less specialized hospitals.

==> macros.tex <==
%% LaTeX macros
\usepackage{times}
%\usepackage{garamond}
%\usepackage{fourier} % math & rm
\usepackage[scaled=1.05]{helvet} % ss
\usepackage{relsize}
\usepackage[dvipsnames]{xcolor}

% Define underscore to be a regular character in text mode
\begingroup
  \catcode`\_=\active
  \gdef_#1{\ensuremath{\sb{#1}}}
\endgroup
\mathcode`\_=\string"8000
\catcode`\_=12

% Set version number
\newcommand\version{$3.2$}

\newcommand\copyrightfootnote{
\footnotetext{Copyright (2008-\the\year{}) of Einar Andreas R{\o}dland, distributed
under the \LaTeX{} Project Public License (LPPL).}
}

%TC:macroword \TeXcount 1
\newcommand\TeXcount{{\TeX}count}

% Text formats
\newcommand\codestyle[1]{\textsf{\color{Blue}#1}}
\newcommand\code[1]{{\smaller\codestyle{#1}}}
\newcommand\bigcode[1]{\codestyle{#1}}
\newcommand\codeline[1]{\begin{quote}\code{#1}\end{quote}}
\newcommand\bs[1]{\textbackslash#1}
\newcommand\URL[1]{\textsf{\small #1}}

% Description items: options, parameters, optional parameters
% These are also interpreted by dos2html.pl
\def\option[#1]{\item[\code{#1}]\hskip 0pt plus 10pt}
\def\parm#1{\textit{\color{OliveGreen}#1}}
\def\opt#1{\parm{[#1]}}
\def\alt#1{[#1]}
\def\optiontext#1{\textrm{\bfseries\color{black}#1}}

% Mark off notification in contents for good visibility
\newcommand\ContentsNote[1]{\addtocontents{toc}{\string\marginpar{\textsf{\color{red}\tiny #1}}}}

% Notabene: margin note
%TC:macro \NB 1
\newcommand\NB[1]{\ContentsNote{NB}\marginpar{\textsf{\tiny#1}}}

% Mark text as a notification
%TC:macro \NOTE [text]
\newcommand\NOTE[1]{\textit{\color{red}#1}}

% Mark text for update
%TC:macro \UPDATE [text]
\newcommand\UPDATE[1]{\ContentsNote{UPDATE}\textit{\textbf{\color{red}This needs to be updated:} {\color{blue}#1}}}

% Mark text as a notification
%TC:macro \TODO [text]
\newcommand\TODO[1]{\ContentsNote{TODO}\textit{\textbf{\color{red}#1}}}

% BUG
%TC:macro \BUG [text]
\newcommand\BUG[1]{{\color{red}#1}}

\makeatletter

\renewcommand\@maketitle{%
\newpage\null\vskip 2em%
\begin{center}%
\let\footnote\thanks
{\LARGE \@title \par}%
\end{center}%
\par
\vskip 1.5em
}

\renewcommand\abstractname{Abstract}
\renewenvironment{abstract}{%
  \begin{center}%
    {\slshape\bfseries\large\abstractname\vspace{-.5em}\vspace{\z@}}%
  \end{center}%
  \vskip 4pt
  \slshape
}{
\vskip 0.5em
}

\makeatother

